Pseudomonads and Descent, PhD Thesis (Chapter 1)

This is the introductory chapter of my PhD Thesis. This thesis consists of one introductory chapter and four single-authored papers written during my PhD studies at the University of Coimbra under supervision of Maria Manuel Clementino. In this first chapter, we give a glance of the scope of our work and briefly describe elements of the original contributions of each paper, including some connections between them. We also give a brief exposition of our main setting, which is $2$-dimensional category theory. In this direction: (1) we give an exposition on the doctrinal adjunction, focusing on the Beck-Chevalley condition as used in Chapter "Pseudo-Kan Extensions and Descent" (arXiv: 1606.04999), (2) we apply the results of "On lifting of biadjoints and lax algebras" (arXiv: 1607.03087) in a generalized setting of the formal theory of monads and (3) we apply the biadjoint triangle theorem of "On biadjoint triangles" (aXiv: 1606.05009) to study (pseudo)exponentiable pseudocoalgebras.

==> thesis-info.tex <==

% ************************ Thesis Information **********************
%% The title of the thesis
\title{Pseudomonads and Descent}

%% The full name of the author
\author{Fernando Lucatelli Nunes}

%% Logo
\crest{\includegraphics[width=0.48\textwidth]{logoUCUP.png}}


%% Full title of the Program
\degree{UC|UP Joint PhD Program in Mathematics \\[3mm] Programa Inter-Universit\'{a}rio de Doutoramento em Matem\'{a}tica \\[15mm]PhD Thesis | Tese de Doutoramento}


%% Submission date
% Default is set as {\monthname[\the\month]\space\the\year}
\degreedate{September 2017}

